Exploring Prompt Engineering Practices in the Enterprise

Interaction with Large Language Models (LLMs) is primarily carried out via prompting. A prompt is a natural language instruction designed to elicit certain behaviour or output from a model. In theory, natural language prompts enable non-experts to interact with and leverage LLMs. However, for complex tasks and tasks with specific requirements, prompt design is not trivial. Creating effective prompts requires skill and knowledge, as well as significant iteration in order to determine model behavior, and guide the model to accomplish a particular goal. We hypothesize that the way in which users iterate on their prompts can provide insight into how they think prompting and models work, as well as the kinds of support needed for more efficient prompt engineering. To better understand prompt engineering practices, we analyzed sessions of prompt editing behavior, categorizing the parts of prompts users iterated on and the types of changes they made. We discuss design implications and future directions based on these prompt engineering practices.

==> todo.tex <==
findings/contributions in intro

methods
    
    


Results
    

    what were other interesting instruction edits
    - TODO: michelle

discussion
    add refs to discussion --- partially done
    add another section to the discussion? -- don't think we actually have space for this
    - TODO: michelle
        try to make the insights more interesting... what hasn't been done? 




Done:
    Mike Change 4.1 to show only the 57 sessions that we analyzed.
        - Revised 4.1
    how many prompts/edits for the 57 sessions (and the six sessions with inter-rating)
        Mike calculate # edits (userid+editid) and add to the methods section
            - Added at the end of section 3.2, number is 1523
    2.29 average number of simultaneous edits-- average of what? 
        - Number of coherent edits (component+edit type) (that we identified) between prompt a and prompt b
            Clarified this statement in the paper, added SD and median

Methods
    Michelle- describe how we got data: by comparing prompt A/prompt B
    also iterated on the description of data collection/sampling. it's quite complicated

Cut: 
    how often did people change between builder and not? 
        - TODO: Calculate how often people switch between the prompt builder

    how big were the different kinds of edits?
        - TODO: Mike Compare task changes to context changes by similarity ratio, report on mean + std

what kinds of edits were rolled back?
what kinds of edits have multiple?

limitations
    - talk about how use cases may skew edit distributions
